Game Theoretic Mixed Experts for Combinational Adversarial Machine Learning

Recent advances in adversarial machine learning have shown that defenses considered to be robust are actually susceptible to adversarial attacks which are specifically customized to target their weaknesses. These defenses include Barrage of Random Transforms (BaRT), Friendly Adversarial Training (FAT), Trash is Treasure (TiT) and ensemble models made up of Vision Transformers (ViTs), Big Transfer models and Spiking Neural Networks (SNNs). We first conduct a transferability analysis, to demonstrate the adversarial examples generated by customized attacks on one defense, are not often misclassified by another defense. This finding leads to two important questions. First, how can the low transferability between defenses be utilized in a game theoretic framework to improve the robustness? Second, how can an adversary within this framework develop effective multi-model attacks? In this paper, we provide a game-theoretic framework for ensemble adversarial attacks and defenses. Our framework is called Game theoretic Mixed Experts (GaME). It is designed to find the Mixed-Nash strategy for both a detector based and standard defender, when facing an attacker employing compositional adversarial attacks. We further propose three new attack algorithms, specifically designed to target defenses with randomized transformations, multi-model voting schemes, and adversarial detector architectures. These attacks serve to both strengthen defenses generated by the GaME framework and verify their robustness against unforeseen attacks. Overall, our framework and analyses advance the field of adversarial machine learning by yielding new insights into compositional attack and defense formulations.

==> GaME E-Print V2/Sections/Attacks.tex <==
\section{New Adversarial Attacks}
\label{sec:attack}
In our paper we assume a white-box adversarial threat model. This means the attacker is aware of the set of all defenses $D$ that the defender may use for prediction. In addition, $\forall d \in D$ the attacker also knows the classifier weights $\theta_{d}$, architecture and  any input image transformations the defense may apply. To generate adversarial examples the attacker solves the following optimization problem:
\begin{equation}
\begin{array}{cc}
    \displaystyle \max_{\delta} \sum_{d \in D} L_{d}(x + \delta, y; d) &  \text{subject to: } ||\delta||_p \leq \epsilon
\end{array}
\label{attackform}
\end{equation}
where $D$ is the set of all possible defenses (models) under consideration in the attack, $L_{d}$ is the loss function associated with defense $d\in D$, $\delta$ is the adversarial perturbation, and $(x,y)$ represents the original input with corresponding class label. This is a more general formulation of the optimization problem allowing the attacker to attack single or multi-model classifiers. The magnitude of this perturbation $\delta$ is typically limited by a certain $l_{p}$ norm. In this paper we analyze the attacks and defenses using the $l_{\infty}$ norm. 

Static white-box attacks such as the Projected Gradient Descent (PGD)~\cite{madry2018towards} attack often perform poorly against randomized defenses such as BaRT or TiT. In~\cite{TiT} they tested the TiT defense against an attack designed to compensate for randomness, the Expectation over Transformation attack (EOT) attack~\cite{EOT}. However, it was shown that the EOT attack performs poorly against TiT (e.g. $20\%$ or worse attack success rate). For attacking BaRT, in~\cite{demystifying} they proposed a new white-box attack to break BaRT. However, this new attack requires that the image transformations used in the  BaRT defense be differentiable, which is a deviation from the original BaRT implementation. 

\textbf{Attack Contributions:} It is crucial for both the attacker and defender to consider the strongest possible adversary when playing the adversarial examples game. Thus, we propose three new white-box attacks for targeting randomized defenses. The first attack is designed to work on single, randomized defenses and is called the Momentum Iterative Method over Expectation (MIME). To the best of our knowledge, MIME is the first white-box attack to achieve a high attack success rate ($>70\%$) against TiT. MIME is also capable of achieving a high attack success rate against BaRT, even when non-differentiable transformations are implemented as part of the defense. Our second attack, is designed to generate adversarial examples that work against multiple type of defenses simultaneously. This compositional attack is called, the Multi-Agent Gradient Expectation attack (MAGE). Lastly, we propose a modified version of MAGE called MAGE-D which is designed to target defenses utilizing consensus voting adversarial detection techniques. MAGE-D is discussed in Section~\ref{sec:GaME}.

\subsection{Momentum Iterative Method over Expectation} %maybe save some lines here?
We develop a new white-box attack specifically designed to work on defenses that inherently rely on randomization, like Barrage of Random Transforms (BaRT)~\cite{BaRT} and Trash is Treasure (TiT)~\cite{TiT}. Our new attack is called the Momentum Iterative Method over Expectation (MIME). The attack ``mimes" the transformations of the defender in order to more precisely model the gradient of the loss function with respect to the input after the transformations are applied. To this end, MIME utilizes two effective aspects from earlier white-box attacks: momentum from the Momentum Iterative Method (MIM)~\cite{MIM} attack, and repeated sampling~\cite{EOT} from the Expectation Over Transformation (EOT) attack:
\begin{equation}
    x^{(i)}_{adv} = x^{(i-1)}_{adv} + \epsilon_{\text{step}} g^{(i)}
    \label{eq:mime}
\end{equation}
where the attack is computed iteratively with $x^{(0)}_{adv}=x$. In Equation~\ref{eq:mime} $g^{(i)}$ is the momentum based gradient of the loss function with respect to the input at iteration $i$ and is defined as:
\begin{equation}
    g^{(i)} := \gamma g^{(i-1)} + \mathbb{E}_{t \sim T}[\frac{\partial L}{\partial t(x^{(i)}_{adv})}]
    \label{eq:MIMEMomentum}
\end{equation}
where $\gamma$ is the momentum decay factor and $t$ is a random transformation function drawn from the defense's transformation distribution $T$. In Table~\ref{tbl:MIME}, we show experimental results for the MIME attack on CIFAR-10 randomized defenses (TiT and BaRT). It can clearly be seen that MIME has a higher attack success rate than both APGD~\cite{APGD} and MIM~\cite{MIM}.

\begin{table}[!h]
\centering

\resizebox{.45\textwidth}{!}{
\begin{tabular}{|c|ccccc|}
\hline
Attack  & BaRT-1          & BaRT-5          & BaRT-10         & TiT (BiT/ViT)  & TiT (VGG/RN) \\ \hline
MIME-10 & \textbf{3.18\%} & 15.5\%          & 43.2\%          & 10.1\%         & 24.9\%            \\
MIME-50 & 4.3\%           & \textbf{8.22\%} & \textbf{23.2\%} & \textbf{8.3\%} & \textbf{23.3\%}   \\
MIM     & 6.7\%           & 39.5\%          & 59.5\%          & 52\%           & 58.9\%            \\
APGD    & 8.9\%           & 47.7\%          & 70.8\%          & 68.2\%         & 40.7\%            \\
Clean   & 98.4\%          & 95.3\%          & 92.5\%          & 90.1\%         & 76.6\%            \\ \hline
\end{tabular}}
\caption{Performance of the MIME attack against CIFAR-10 randomized defenses TiT and BaRT with $\epsilon_{max}=0.031$. It can clearly be seen that MIME outperforms both APGD and MIM on these two randomized defenses. Full experimental details are given in the supplemental material.}
\label{tbl:MIME}
\end{table}

\subsection{Multi-Agent Gradient Expectation attack}

%Much of the adversarial machine learning literature has focused on single model attacks (e.g. FGSM, MIM, PGD, APGD, etc.). Multi-model attacks on vanilla (undefended) CNN models may not have received as much attention, due in part to the transferability of adversarial examples. To clarify, adversarial examples generated from one CNN are often misclassified by other CNNs, even when the CNNs have different architectures or training~\cite{Delving}. Multi-model attacks are simply unnecessary when single model attacks transfer well between multiple CNN models.

The use of multi-model attacks are necessary to achieve a high attack success rate when dealing with ensembles that contain both CNN and non-CNN model architectures, like the Vision Transformer (ViT)~\cite{VIT} and Spiking Neural Network (SNN)~\cite{SEW}. This is because adversarial examples generated by single model white-box attacks generally do not transfer well between CNNs, ViTs and SNNs~\cite{mahmood2021robustness, xu2022securing}. In addition it is an open question if multi-model attacks can be effective against the current state-of-the-art defenses. In this paper, we expand the idea of a multi-model attack to include not only different architecture types, but also different defenses. The generalized form of the multi-model attack is found in Equation~\ref{attackform}.

For a single input $x$ with corresponding class label $y$, an untargeted multi-model attack is considered successful if $(\forall d \in D, C_{d}(x+\delta) \neq y) \land (||\delta||_p \leq \epsilon)$. One formulation of the multi-model attack is the Auto Self-Attention Gradient Attack (Auto SAGA)~\cite{xu2022securing}. Auto SAGA iteratively attacks combinations of ViTs, SNNs and CNNs:
\begin{equation}
    x_{adv}^{(i+1)} = x_{adv}^{(i)} + \epsilon_{step}*\text{sign}(
    G_{blend}(x_{adv}^{(i)}))
    \label{eq:sagamain}
\end{equation}
where $\epsilon_{step}$ was the step size used in the attack. In the original formulation of Auto SAGA, $G_{blend}$ was a weighted average of the gradients of each model $d \in D$. By combining gradient estimates from different models, Auto SAGA is able to create adversarial examples that are simultaneously misclassified by multiple models. One limitation of Auto SAGA attack is that it does not account for defenses that utilize random transformations. Motivated by this, we can integrate the previously proposed MIME attack into the gradient calculations for Auto SAGA. We denote this new attack as the Multi-Agent Gradient Expectation attack (MAGE). Both SAGA and MAGE use the same iterative update (Equation~\ref{eq:sagamain}). However, MAGE uses the following gradient estimator:
\begin{equation}
    {\small
    \begin{array}{c}
         \displaystyle G_{blend}(x_{adv}^{(i)}) = \gamma G_{blend}(x_{adv}^{(i-1)}) + \sum_{k \in D \backslash R} \alpha^{(i)}_{k} \phi^{(i)}_{k} \odot \frac{\partial L_{k}}{\partial x_{adv}^{(i)}}  \\
         \displaystyle + \sum_{r \in R} \alpha^{(i)}_{r} \phi^{(i)}_{r} \odot (\mathbb{E}_{t \sim T}[\frac{\partial L_{r}}{\partial t(x^{(i)}_{adv})}])
    \end{array}}
    \label{eq:ae}
\end{equation}
In Equation~\ref{eq:ae}, the two summations represent the gradient contributions of sets $D \backslash R$ and $R$, respectively. Here we define $R$ as the set of randomized defenses and $D$ as the set of all the defenses being targeted. In each summation $\phi$ is the self-attention map~\cite{abnar2020quantifying} which is replaced with a matrix of all ones for any defense that does not use ViT models. $\alpha_{k}$ and $\alpha_{r}$ are the associated weighting factors for the gradients for each deterministic defense $k$ and randomized defense $r$, respectively. Details of how the weighting factors are derived are given in~\cite{xu2022securing}. We further develop this  attack formulation into a novel attack (MAGE-D) that is effective on detection based defenses in Section~\ref{sec:GaME}. Experimental results for both MAGE and MAGE-D are give within Section~\ref{sec:exp}.

%The last summation of Equation~\ref{eq:ae} represents the approximated gradient contribution on a randomized defense where $t$ is a random transformation function sampled from the defense's transformation distribution $T$.

% This composition of gradient estimators creates a new attack capable of generating adversarial examples for a combination of defenses that use either CNNs, ViTs, SNNs and/or defenses which incorporate randomization.

%Note $V \cap R, \; K \cap R \neq \emptyset$ when there is a randomized defense with a ViT or CNN classifier respectively.
%The difference between SAGA and MAGE lies in the segmentation of defenses. We can further specify the set of all defenses (models) as $D=K \cup R$, where $K$ represents the set of all defenses using CNN models and $R$ represents the set of all defenses using randomized models.

%G_{blend}(x_{adv}^{(i)}) = \sum_{k \in K} \alpha_{k} \frac{\partial L_{k}}{\partial x_{adv}^{(i)}} + \sum_{v \in V} \alpha_{v} \phi_{v} \odot \frac{\partial L_{v}}{\partial x_{adv}^{(i)}} + \sum_{r \in R} \alpha_{r} (\gamma g^{(i-1)}_{r} + \mathbb{E}_{t \sim T}[\frac{\partial L_{r}}{\partial t(x^{(i)}_{adv})}])

%where $\epsilon_{\text{step}}$ is the step size of the attack, $\alpha_i^c$ a weighting matrix, and $\phi^c$ is the self attention rollout. The values for $\alpha_i^c$ and $\phi^c$ are highly important to the attack's success and are automatically computed by the algorithm. In~\cite{xu2022securing} explicit formulas for these calculations are provided.

%One limitation of Auto-SAGA attack is that it does not account for defenses that utilize random transformations. Motivated by this, we have built upon Auto-SAGA by building MIME into the attack's gradient calculation. The attack update step for this modified version of the attack, MAGE is as follows:

%\begin{equation}
%    G_i^{\text{blend}} = \gamma G_{i-1}^{\text{blend}} + \text{sign}(\displaystyle \sum_j^N ( \sum_{c \in C} \alpha_{i-1}^c \odot \frac{\partial L_c}{\partial t^c_j(x^{adv}_{i-1})} \odot \phi_c ))
%\end{equation}


%In~\cite{xu2022securing} the Auto Self Attention Gradient Attack (Auto-SAGA) was proposed as a new algorithm for attacking an ensemble of defenses, $C$. The attack tries to maximize the loss of each model within the ensemble by using a weighted summation of their gradient vectors with respect to the input. Thus it solves the following optimization problem:

%In addition to considering the gradient of each model in the ensemble, Auto-SAGA also targets Vision Transformers by utilizing their attention weight matrix at each attention head in the gradient calculation. At each attack step the adversarial example $x^{adv}$ is updated as follows:
%\begin{equation}
%    x^{adv}_i = x^{adv}_{i-1} + \epsilon_{\text{step}} \cdot \text{sign}( \sum_{c \in C} \alpha_{i-1}^c \odot \frac{\partial L_c}{\partial x^{adv}_{i-1}} \odot \phi_c )
%\end{equation}



%Need to figure out citing section
%Similar to MIME we take $N$ Monte-Carlo samples to approximate the gradient of the loss function with respect to $t(x^{adv}_{i})$. For defenses that have no transformation $t$ is set to be the identity function and $N$ is set to $1$. While integrating MIME does increase the computational complexity of the attack, it allows us to craft a stronger attack for targeting ensembles of random transformation defenses and deterministic defenses. As previously mentioned, this is critical for both the defender and attacker in the adversarial game developed in the next section.


%the attacker has white box access to each of the defender's classifiers. This means the attacker can utilize information about each defenses' architecture, trained weights, and random transformations in order to craft adversarial examples. When generating adversarial examples the attacker tries to solve the following optimization problem:

%\begin{equation}
 %   \begin{array}{c c}
 %   \displaystyle \max_{\delta} \mathbb{P}(C(x + \delta) \neq %y) &  \text{subject to: } ||\delta||_p \leq \epsilon
%end{array}
%\end{equation}

%where $C$ is some classifier function, $x$ is an unperturbed input to the classifier, $y$ is the ground truth class label for $x$, and $\epsilon$ is a parameter limiting the size of the attacker's perturbation vector, $\delta$. The optimization problem is difficult to solve in this form, thus many attacks are designed to maximize the model's loss with respect to some loss function $L$:



%In this paper we propose two new versions of exisiting attacks: MIME, an improved version of MIM utilizing EOT, and MAGE, a version of Auto-SAGA utilizing momentum and EOT. Both of these attacks utilize EOT to target random transform defenses which are otherwise very robust against white box attacks. They also employ momentum, which was shown in (cite BARZ + ICCV) to increase attack transferability between different models. Transferability is important as the attacker will be trying to break an ensemble of defenses.

%Developing attacks which target or break certain defenses is critical to the Game Theory section of this paper as omitting sufficiently strong attacks will give a false sense of robustness to certain defenses in an ensemble. This will lead these defenses to be over-represented in the ensemble's probability distribution despite their weakness. 


%Many defenses such as BaRT and TiT utilize random, often non-differentiable transformations to increase their robustness. These defenses are very strong against black box attacks as well as white box attacks which do not take their random transformations into consideration. In~\cite{demystifying} the strength of these defenses was explored in more detail. In particular, they developed new attacks and defenses which hinge upon the defender using differentiable transformations in a predetermined order. This enables the attacker to propagate the gradient of the loss with respect to the input through the transformation functions, allowing them to craft stronger adversarial examples.


%In this work we assume the defender does not give the attacker the benefit of differentiable transformations, and further uses a random transformation order. This generally makes for a stronger, albeit harder to analyze, defense. Thus, in order to successfully attack the BaRT and TiT defenses we develop a new attack, Momentum Iterative Method over Expectation (MIME). This attack combines ideas from~\cite{MIM} and~\cite{EOT} to create a momentum based, EOT attack. The attack ``mimes" the transformations of the defender in order to get a better idea of the gradient of the loss function with respect to the input after the transformations are applied. The attack is iterative and applies the following attack update:
%\begin{equation}
 %   x^{adv}_i = x^{adv}_{i-1} + \epsilon_{\text{step}} G_i
%\end{equation}
%where $G_i$ is the momentum based gradient of the loss function with respect to the input at time step $i$ and is updated as follows:
%Need stuff to notate xadv being projected back within epsilon
%\begin{equation}
%    G_i := \gamma G_{i-1} + \mathbb{E}_{t \sim T}[\frac{\partial L}{\partial t(x^{adv}_i)}]
%\end{equation}
%where $\gamma$ is the momentum decay factor and $t$ is a random transformation function drawn from the defense's transformation distribution $T$. In practice $G_i$ is approximated using $N$ Monte Carlo samples per input $x$:
%\begin{equation}
%    G_i \approx \gamma G_{i-1} + (\frac{1}{N} \displaystyle\sum_{i=0}^N \frac{\partial L}{\partial t_i(x^{adv}_i)})
%\end{equation}
%Flesh out more
%The MIME attack is able to out perform the standard MIM and Auto-PGD attacks which do not use EOT techniques \ref{MIME}. In addition to this, MIME is able to break both versions of the Trash is Treasure defense that we implemented. 

%Transpose table
%\begin{table}[!h]
%    \centering
%    \begin{tabular}{|c| c c c c c|}
%        \hline Defense & MIME-10 & MIME-50 & MIM & APGD & Clean \\ \hline
%        BaRT-1 & 3.18\% & 4.3\% & 6.7\% & & 98.4\% \\
%        BaRT-5 & 15.5\% & 8.22\% & 39.5\% & & 95.3\% \\
%        BaRT-10 & 43.2\% & 23.2\% & 59.5\% & & 92.5\% \\
%        TiT (BiT+ViT) & 10.1\% &  & 52\% & &  90.1\% \\
%        TIT (VGG + ResNet) & 24.9\% & 23.3\% & 58.9\% & & 76.6\% \\ \hline
%    \end{tabular}
%    \caption{\centering (CIFAR-10, $\epsilon = .031$) Performance of MIME against random transform defenses compared to images generated by the standard MIM attack and APGD. MIME(n) represents an instance of MIME where n samples are taken in the gradient approximation.}
%    \label{MIME}
%\end{table}
%From a game theoretic perspective, and when compared against the alternative strategies of using APGD or MIM, MIME can be seen as a best response strategy against a defender who chooses to use a TiT or BaRT defense strategy. 


%\subsection{Auto-PGD}

%Auto-PGD is an attack proposed in~\cite{APGD} to be a modified version of the PGD attack~\cite{madry2018towards} with an automatically calculated attack step size, $\epsilon_{\text{step}}$. We have chosen to include this attack in our paper since it is a more effective replacement for PGD or MIM when attacking defenses without random transforms. APGD also implements momentum into its gradient calculation, allowing for a possible increase in transferability as explored in (CITE BARZ AND ICCV PAPER).

==> GaME E-Print V2/Sections/Conclusion.tex <==
\section{Conclusion}
The field of adversarial machine learning has begun to cycle between new defenses, specialized attacks to break those defenses, and further specialized defenses to mitigate the attacks. In this paper, we seek to go beyond this cat and mouse dynamic by considering a new game theoretic framework that incorporates multiple defenses, adversarial detection, and compositional attacks.

We develop three new white-box attacks, the Momentum Iterative Method over Expectation (MIME) for attacking single randomized defenses and the Multi-Agent Gradient Expectation attacks (MAGE and MAGE-D) for dealing with a combination of randomized and non-randomized defenses and detectors. Additionally, we are the first to show the transferability of adversarial examples generated by MIM, APGD, MIME and MAGE on state-of-the-art defenses like FAT, BaRT and TiT. 

Lastly, and most importantly, we develop a game theoretic framework to approximate an optimal strategy for adversarial attackers and defenders. The flexibility of this framework allows any newly proposed defense or attack to be easily integrated. Using a set of SOTA attacks and defenses we demonstrate that our game theoretic framework can create a compositional defense that achieves a 37.3\% and 45.65\% increase in robustness on Tiny ImageNet and CIFAR-10 respectively when utilizing a mixed Nash strategy (compared to using the best single defense). Both compostional GaME defenses also come with higher a clean accuracy than the most robust, single model defenses.

==> GaME E-Print V2/Sections/Defenses.tex <==
\section{Adversarial Machine Learning Defenses}

In the following subsections, we give an overview of each defense and our reasons for choosing said defense. It is important to note our analyses encompass a broad range of different defenses, including ones based on randomization, ones based on adversarial training and ones based on exploiting model transferability. In addition, we also consider diverse architectures including Big Transfer models (BiTs), Vision Transformers (ViTs) and Spiking Neural Networks (SNNs). Despite our broad range, we do not attempt to test every novel adversarial defense. It is simply infeasible to test every proposed adversarial machine learning defense, as new defenses are constantly being produced. Corresponding code to replicate our results can be found \href{https://github.com/EthanRath/Game-Theoretic-Mixed-Experts}{here}.  

\subsection{Barrage of Random Transforms} %BaRT ref

Barrage of Random Transforms (BaRT)~\cite{BaRT} utilize a set of image transformations in a random order and with randomized transformation parameters to thwart adversarial attacks. In this paper, we work with the original BaRT implementation which includes both differentiable and non-differentiable image transformations.


%Let $t^{i}_{j}(x)$ represent the $i^{th}$ transformation used in the $j^{th}$ order in the sequence. A BaRT defense using $n$ image transformations randomly alters the input $x$:
%\begin{equation}
 %   t(x)=t^{\omega_{n}}_{\mu_{n}} \circ t^{\omega_{n-1}}_{\mu_{n-1}} \circ ...\circ %t^{\omega_{1}}_{\mu_{1}}(x)
    \label{eq:bart}
%\end{equation}
%where $\omega$ represents the subset of $n$ transformations randomly selected from a set of $N$ total possible transformations and $\mu$ represents the randomized order in which the $n$ transformations are applied. In Equation~\ref{eq:bart} the parameters of each image transformation $t^{i}_{j}(x)$ are also randomized at run time, further adding to the stochastic nature of the defense. In this paper, we work with the original BaRT implementation which includes both differentiable and non-differentiable image transformations. %Full defense and transformation implementation details for our BaRT models are given in the supplementary material. 

\textbf{Why we selected it:} Many defenses are broken soon after being proposed~\cite{tramer2020adaptive}. BaRT is one of the few defenses that has continued to show robustness even when attacks are specifically tailored to work against it. For example, most recently BaRT achieves $29\%$ robustness on CIFAR-10 against a customized white-box attack~\cite{demystifying}. It remains an open question whether using BaRT with other randomized approaches (i.e. selecting between different defenses) can yield even greater robustness.

\subsection{Friendly Adversarial Training} %FAT ref

Training classifiers to correctly recognize adversarial examples was originally proposed in~\cite{goodfellow2014explaining} using FGSM. This concept was later expanded to include training on adversarial examples generated by PGD in~\cite{madry2018towards}. In~\cite{FAT}, it was shown that Friendly Adversarial Training (FAT) could achieve high clean accuracy, while maintaining robustness to adversarial examples. This training was accomplished by using a modified version of PGD called PGD-$K$-$\tau$. In PGD-$K$-$\tau$, $K$ refers to the number of iterations used for PGD. The $\tau$ variable is a hyperparamter used in training which stops the PGD generation of adversarial examples earlier than the normal $K$ number of steps, if the sample is already misclassified.     

\textbf{Why we selected it:} There are many different defenses that rely on adversarial training~\cite{madry2018towards, zhang2019theoretically, wang2019improving, maini2020adversarial} and training and testing them all is not computationally feasible. We selected FAT for its good trade off between clean accuracy and robustness, and because we wanted to test adversarial training on both Vision Transformer and CNN models. In this regard, FAT is one of the adversarial training methods that has already been demonstrated to work across both types of architectures~\cite{mahmood2021robustness}. 


%\begin{equation}
%\min_{f \in F} \frac{1}{n} \sum^{n}_{i=1} %l(C(x^{adv}_{i}),y_{i})
%\end{equation}

\subsection{Trash is Treasure} %TiT ref

One early direction in adversarial defense design was  model ensembles~\cite{pang2019improving}. However, due to the high transferability of adversarial examples between models, such defenses were shown to not be robust~\cite{tramer2020adaptive}. Trash is Treasure (TiT)~\cite{TiT} is a two model defense that seeks to overcome the transferability issue by training one model $C_{a}(\cdot)$ on the adversarial examples from another model $C_{b}(\cdot)$. At run time both models are used:
\begin{equation}
    y = C_{a}(\psi(x, C_{b}))
\end{equation}
where $\psi$ is an attack done on model $C_{b}$ with input $x$ and $C_{a}$ is the classifier that makes the final class label prediction on the adversarial example generated by $\psi$ with $C_{b}$.

\textbf{Why we selected it:} TiT is one of the newest defenses that tries to achieve robustness in a way that is fundamentally different than pure randomization strategies or direct adversarial training. In our paper, we further develop two versions of TiT. One version is based on the original proposed CNN-CNN implementation. We also test a second mixed architecture version using Big Transfer model and Vision Transformers to try and leverage the low transferability phenomena described in~\cite{mahmood2021robustness}.    

\subsection{Novel Architectures} %SEW ref for SNN

In addition to adversarial machine learning defenses, we also include several novel architectures that have recently achieved state-of-the-art or near state-of-the-art performance in image recognition tasks. These include the Vision Transformer (ViT)~\cite{VIT} and Big Transfer models (BiT)~\cite{BIT}. Both of these types of models utilize pre-training on larger datasets and fine tuning on smaller datasets to achieve high fidelity results. We also test Spiking Neural Network (SNNs) architectures. SNNs are a competitor to artificial neural networks that can be described as a linear time invariant system with a network structure that employs non-differentiable activation functions~\cite{xu2022securing}. A major challenge in SNNs has been matching the depth and model complexity of traditional deep learning models. Two approaches have been used to overcome this challenge, the Spiking Element Wise (SEW) ResNet~\cite{SEW} and transferring weights from existing CNN architectures to SNNs~\cite{rathi2021diet}. We experiment with both approaches in our paper.  

\textbf{Why we selected it:} The set of adversarial examples used to attack one type of architecture (e.g. a ViT) have shown to not be misclassified by other architecture types (e.g. a BiT or SNN)~\cite{mahmood2021robustness, xu2022securing}. While certain white-box attacks have been used to break multiple undefended models, it remains an open question if different architectures combined with different defenses can yield better performance.  

%In our framework the defender has access to a set of adversarial defense classifiers, $D$. When the defender receives an input, $x$, they can then chose a random subset, $U \subset D$ with which to make the final classification according to some decision function

==> GaME E-Print V2/Sections/ExperimentsGame.tex <==
\section{Experimental Results} \label{sec:exp}
\begin{figure}
\centering
\subfloat[CIFAR-10]{%
  \includegraphics[clip,width=.9\columnwidth]{Figures/barcifar.pdf}%
}

\subfloat[Tiny ImageNet]{%
  \includegraphics[clip,width=0.9\columnwidth]{Figures/bartiny.pdf}%
}
\caption{Comparison of GaME ensembles to the three most robust, single-model defenses for each dataset. and GaME ensemble results.}
\label{bars}
\end{figure}
 We test on two datasets for our experimental results, CIFAR-10~\cite{c10} and Tiny ImageNet~\cite{le2015tiny}. For CIFAR-10 we solved instances of $\text{GaME}_n$ using the following defenses: BaRT-1 (B1), BaRT-5 (B5), ResNet-164-FAT (RF), ViT-L-16-FAT (VF), SNN Transfer (ST), Backprop SNN (SB), and TiT using ViT and BiT (BVT). For Tiny ImageNet we solved instances of $\text{GaME}_n$ utilizing: BaRT-1, BaRT-5, ViT-L-16-FAT, and TiT using ViT and BiT. Explicit details for our experimental setup are given in the supplementary material.
 
In Figure~\ref{bars} and throughout the paper, we measure the robustness of each ensemble as the lowest robust accuracy achieved by any single attack in our study. From a game-theoretic perspective this can be seen as the minimum, guaranteed utility for the defender. Of all the defenses in our study the FAT ResNet-164 had the highest robust accuracy on CIFAR-10 at 45\%. On Tiny ImageNet, BaRT-5 had the highest robust accuracy at 11\%. Compared to these defenses our GaME generated ensemble achieved 63\% robustness on CIFAR-10 and 24.5\% robustness on Tiny ImageNet without using detectors. When detectors were implemented this increased to to 82.31\% robustness and 57.40\% robustness on each respective dataset.

Additionally, our ensemble is able to maintain a high level of clean accuracy. In particular, the GaME framework maintains 96.2\% clean accuracy on CIFAR-10 and 72.6\% clean accuracy on Tiny ImageNet without detectors. This is only out performed by BaRT-1 with a clean accuracy of 98.4\% on CIFAR-10 and the BiT-ViT Trash is Treasure defense with a clean accuracy of 76.97\% on Tiny ImageNet. With detectors the clean accuracy dropped to 82.9\% and 67.3\% respectively. It is important to note that in both these cases the robustness of the GaME framework is much higher both with and without adversarial detection. We provide more detailed, numerical results for these figures in the supplementary material. Additionally, we provide studies of the effects of $n$ (the maximum ensemble size) and $N$ (the sample number) on $\text{GaME}_n$ generated ensembles along with an analysis of the computational cost of the framework. Lastly, we include studies comparing the effectiveness of the GaME framework to naive ensemble defenses utilizing a uniform distribution over all strategies. 

%\begin{figure*}[h]
%\centering
%\begin{minipage}{.45\linewidth}
%  \centering
%    \includegraphics[width=\linewidth]{Figures/barcifar.pdf}
%    \captionsetup{type=figure}
%\end{minipage}
%\begin{minipage}{.45\linewidth}
%  \centering
%    \includegraphics[width=\linewidth]{Figures/bartiny.pdf}
%    \captionsetup{type=figure}
%\end{minipage}
%\caption{(Left: CIFAR-10; Right: Tiny ImageNet) Comparison of the robust and clean accuracy of the top three most robust single model defenses to three GaME generated ensembles on CIFAR-10 and Tiny ImageNet.}
%\label{fig:results}
%\end{figure*}

==> GaME E-Print V2/Sections/ExperimentsTransfer.tex <==
\section{Transferability Experiments}
\label{sec:trans}
\begin{table}
    \centering
    \resizebox{.8\linewidth}{!}{
    \begin{tabular}{|c|ccc|}
            \hline
            Defense & Best Attack & Clean Acc & Robust Acc \\ \hline
            B1      & MIME        & 98.40\%   & 3.40\%     \\ \hline
            B5      & MIME        & 95.30\%   & 15.00\%    \\ \hline
            B10     & MIME        & 92.50\%   & 43.50\%    \\ \hline
            RF      & APGD        & 81.89\%   & 52.00\%    \\ \hline
            VF      & APGD        & 92.36\%   & 25.00\%    \\ \hline
            ST      & APGD        & 91.54\%   & 0.00\%     \\ \hline
            SB      & APGD        & 81.16\%   & 1.60\%     \\ \hline
            BVT     & MIME        & 90.10\%   & 8.60\%     \\ \hline
            VRT     & MIME        & 76.60\%   & 26.20\%    \\ \hline
        \end{tabular}}
        \caption{Single defense implementations for CIFAR-10 with the corresponding strongest attack on the defense and the clean accuracy of the defense. All attacks are done with $\epsilon_{max}=0.031$. Complete attack and defense implementation details are given in our supplementary material.}
        \label{tbl:bestAttack}
\end{table}
\begin{figure}
    \centering
    \includegraphics[width=60mm]{Figures/Figure_1.pdf}
    \captionsetup{type=figure}
    \caption[]{Visual representation of the transferability of adversarial examples between defenses for CIFAR-10. A higher bars means more adversarial examples are misclassified. Full numerical tables for the figure are given in our supplemental material.}
    \label{fig:transferability}
\end{figure}
Adversarial transferability refers to the phenomena in which adversarial examples generated to attack one model are also misclassified by a different model. Adversarial transferability studies have been done on a variety of machine learning models~\cite{Delving, mahmood2021robustness, xu2022securing}. However, to the best of our knowledge, adversarial transferability between different state-of-the-art defenses has not been conducted. This transferability property is of significant interest because a lack of transferability between different defenses may indicate a new way to improve adversarial robustnes. 

In Table~\ref{tbl:bestAttack}, we show the different single defenses we analyze in this paper and the best single attack on each of them from the set of attacks (MIM~\cite{MIM}, APGD~\cite{APGD} and MIME (proposed in this work). In Figure~\ref{fig:transferability}, we visually show the transferability results of these attacks for CIFAR-10. The blue bars represent the transferability of adversarial examples generated using the best attack for BaRT models, the green bars represent adversarial examples generated using  the best attack for TiT, the pink bars represent the adversarial examples generated using the best attack for FAT and lastly the purple bars represent the adversarial examples generated using SNNs. We give detailed discussions of these results in our supplementary material and briefly summarize of the key takeaways from these experiments.

Adversarial examples generated using the best attack on one defense \textit{did not} transfer well to other defenses. For example, only $0.8\%$ of the adversarial examples generated by the BaRT-1 defense transfer to the FAT ViT defense. The average transferability for the 8 different defenses shown in Figure~\ref{fig:transferability} is only $21.62\%$ and there is no single model attack that achieves strong performance (i.e. $>50\%$) across all defenses. These results in turn motivate the development of a game theoretic framework for both the attacker and defender. For the attacker, this prompts the need to use multi-model attack like MAGE that was proposed in Section~\ref{sec:attack}, as no single attack (APGD, MIM or MIME) is ubiquitous. For the defender, these results highlight the opportunity to increase robustness by taking advantage of the low levels of transferability between defenses through the implementation of a randomized ensemble defense.
% \begin{table*}
% 	\begin{minipage}{0.47\linewidth}
% 		\centering
% 		\begin{tabular}{|c|ccc|}
%             \hline
%             Defense & Best Attack & Clean Acc & Robust Acc \\ \hline
%             B1      & MIME        & 98.40\%   & 3.40\%     \\ \hline
%             B5      & MIME        & 95.30\%   & 15.00\%    \\ \hline
%             B10     & MIME        & 92.50\%   & 43.50\%    \\ \hline
%             RF      & APGD        & 81.89\%   & 52.00\%    \\ \hline
%             VF      & APGD        & 92.36\%   & 25.00\%    \\ \hline
%             ST      & APGD        & 91.54\%   & 0.00\%     \\ \hline
%             SB      & APGD        & 81.16\%   & 1.60\%     \\ \hline
%             BVT     & MIME        & 90.10\%   & 8.60\%     \\ \hline
%             VRT     & MIME        & 76.60\%   & 26.20\%    \\ \hline
%         \end{tabular}
%         \caption{Single defense implementations for CIFAR-10 with the corresponding strongest attack on the defense and the clean accuracy of the defense. All attacks are done with $\epsilon_{max}=0.031$. Complete attack and defense implementation details are given in our supplementary material.}
%         \label{tbl:bestAttack}
% 	\end{minipage}\hfill
% 	\begin{minipage}{0.47\linewidth}
% 		\centering
% 		\includegraphics[width=65mm]{Figures/Figure_1.pdf}
% 		\captionsetup{type=figure}
% 		\caption[]{Visual representation of the transferability of adversarial examples between defenses for CIFAR-10. A higher bars means more adversarial examples are misclassified. Full numerical tables for the figure are given in our supplemental material.}
%         \label{fig:transferability}
% 	\end{minipage}
% \end{table*}

%The robust accuracy is measured using 1000 adversarial examples. The examples are class wise balanced and also correctly recognized by all the defenses in their original clean form.

%Visual representation of the transferability of adversarial examples between defenses for CIFAR-10. The blue bars represent the transferability of adversarial examples generated using the best attack for BaRT models, the green bars represent adversarial examples generated using  the best attack for TiT, the pink bars represent the adversarial examples generated using the best attack for FAT and lastly the purple bars represent the adversarial examples generated using SNNs. Higher bars means more of the adversarial examples are misclassified by other defenses. Full numerical tables used to generate this figure are given in our supplemental material.

==> GaME E-Print V2/Sections/Game.tex <==
\section{Game theoretic Mixed Experts (GaME)}
\label{sec:GaME}
In this section we derive our framework, Game theoretic Mixed Experts (GaME), for approximating a Nash equilibrium in the adversarial examples game. In comparison to other works \cite{meunier2021mixed} \cite{pinot2020randomization} \cite{pal2020game} \cite{balcan2022nash} \cite{pmlr-v151-le22c} we take a more discretized approach and solve the approximate version of the adversarial examples game. This ultimately leads to the creation of a finite, tabular, zero-sum game that can be solved in polynomial time using linear programming techniques.
\subsection{The Adversarial Examples Game}
We build upon and discretize the adversarial examples game explored in~\cite{meunier2021mixed}. The adversarial examples game is a zero-sum game played between two players: the attacker, $p_A$, and the defender $p_D$. Let $\mathcal{X}$ be the input space and $\mathcal{Y}$ the output space of $p_D$'s classifiers, and let $\Theta$ represent the space of classifier parameters. Additionally, let $P_{\epsilon, \mathcal{X}} = \{x \in \mathcal{X} : ||x||_p \leq \epsilon \}$ be the set of valid adversarial perturbations for norm $p$ and $\epsilon \in \mathbb{R}^+$.
Let $A^*_\epsilon = \{(f : \Theta \times \mathcal{X} \times \mathcal{Y} \rightarrow P_{\epsilon, \mathcal{X}})\}$ be the set of all valid attack functions. The goal of $p_A$ is to choose $a \in A^*_\epsilon$, which maximizes the expected loss of $p_D$'s classifier, $\theta$, given some pair of input and ground truth label $(x,y) \in \mathcal{X} \times \mathcal{Y}$. The goal of $p_D$ is to minimize this loss through its choice of $\theta \in \Theta$. We can thus formulate the adversarial examples game as a mini-max optimization problem:
\begin{equation}
    \displaystyle \inf_{\theta \in \Theta} \sup_{a \in A^*_\epsilon} \E_{(x,y) \sim \mathcal{X} \times \mathcal{Y}} [L(x + a(\theta ,x,y), y ; \theta)]
\end{equation}
Due to the vastness of $\Theta$ and $A^*_\epsilon$, solving this optimization problem directly is currently computationally intractable. To this end, in the next subsections we will formulate $\text{GaME}_1$ and $\text{GaME}_n$ which discretize $\Theta$ and $A^*_\epsilon$ by enlisting a set of state-of-the-art attacks and defenses. 
\subsection{$\textbf{GaME}_1$}
The goal of the GaME framework is to find an approximate solution to the adversarial examples game through the implementation of a set of attacks and defenses which will serve as experts for $p_A$ and $p_D$. Let $A'  \subset  A^*_\epsilon$ be a subset of all valid adversarial attack functions chosen by $p_A$. Additionally, let $D \subset \Theta$ be a set of defense classifiers chosen by $p_D$. We further impose that all $a\in A'$ are white-box attacks (see Section~\ref{sec:attack} for our adversarial threat model) and that $A',D$ are finite, i.e. $|A'| \leq N_a$ and $|D| \leq N_d$ for some $N_a, N_d \in \mathbb{N}$. It is important to note that each $a \in A'$ is a function of some classifier, $\theta \in \Theta$, in addition to the input and ground truth label. Due to this it is possible for $p_A$ to chose to attack defense $d \in D$ with attack $a \in A'$, while $p_D$ chooses to evaluate the sample using defense $d' \in D$ where $d \neq d'$. Therefore, for convenience, we will define a new, more general set of attack strategies for $p_A$:
\begin{equation}
    \begin{array}{c}
         A \subseteq \{ (f : \mathcal{X} \times \mathcal{Y} \rightarrow P_{\epsilon, \mathcal{X}}) : \\ 
         f(x,y) = a_i(U, x, y), \; a_i \in A', \; U \subseteq D \}  
    \end{array}
\end{equation}
where we extend the definition of $A'\subseteq A^*_\epsilon$ to attack functions, such as MAGE, that can take subset of defense parameters $U\subseteq D$ as input (see Equation~\ref{attackform} for our multi-model attack formulation). Thus we will let $D$ be the strategy set of $p_D$, and $A$ be the strategy set of $p_A$. We can then formulate a discretized version of the adversarial examples game as follows:
\begin{equation}
    \displaystyle \min_{d \in D} \max_{a \in A} \E_{(x,y) \sim \mathcal{X} \times \mathcal{Y}}[L(x + a(x,y), y ; d)]
\end{equation}
In the above two formulations we optimize over the set of pure strategies for the attacker and defender. However, as previously explored in~\cite{araujo2020advocating}~\cite{meunier2021mixed}, limiting ourselves to pure strategies severely inhibits the strength of both the attacker and defender. Thus we create the following mixed strategy vectors for $p_A$, $p_D$:
\begin{equation}
\begin{array}{c}
    \lambda^A \in \{r \in [0,1]^{|A|} : ||r||_1 = 1\} \\    \lambda^D \in \{r \in [0,1]^{|D|} : ||r||_1 = 1\}
\end{array}
\end{equation}
here $\lambda^A$ and $\lambda^D$ represent the mixed strategies of $p_A$ and $p_D$ respectively. Let each $a_i \in A$ and $d_i \in D$ correspond to the $i^{th}$ elements of $\lambda^A$ and $\lambda^D$, $\lambda^A_i$ and $\lambda^D_i$, respectively.
\begin{equation}
    \mathbb{P}(\{a_i \in A : a = a_i\}) = \lambda^A_i, \;  
    \mathbb{P}(\{d_i \in D : d = d_i\}) = \lambda^D_i
\end{equation}
where $a \in A$ and $d \in D$ are random variables. With these mixed strategy vectors we can then reformulate the adversarial examples game as a mini-max optimization problem over $p_D$'s choice of $\lambda^D$ and $p_A$'s choice of $\lambda^A$:
\begin{equation}
{\small
\begin{array}{c}
    \displaystyle \min_{\lambda^D} \max_{\lambda^A} \E_{(x,y) \sim \mathcal{X} \times \mathcal{Y}}[ \E_{(a,d) \sim A \times D} [L(x + a(x,y), y ; d)]] =  \\
    \displaystyle  \min_{\lambda^D} \max_{\lambda^A} \E_{(x,y) \sim \mathcal{X} \times \mathcal{Y}}[ \sum_{a_i \in A} \lambda^A_i 
    \displaystyle \sum_{d_i \in D} \lambda^D_i [L(x + a_i(x,y), y ; d_i)]]
\end{array}}
\end{equation}
For continuous and or non-finite $\mathcal{X}$, $D$, and $A$ solving the above optimization problem is currently computationally intractable. Thus, we can instead approximate the mini-max optimization by taking $N$ Monte-Carlo samples with respect to $(x_j,y_j) \in \mathcal{X} \times \mathcal{Y}$:
{\small \begin{equation}
   \displaystyle  \min_{\lambda^D} \max_{\lambda^A} \frac{1}{N}\sum_{j=0}^N \sum_{a_i \in A} \lambda^A_i \sum_{d_i \in D} \lambda^D_i [L(x_j + a_i(x_j,y_j), y_j ; d_i)]
\end{equation}}
For convenience we denote $r_{d_i, a_i} = \frac{1}{N}\sum_{j=0}^N [L(x_j + a_i(x_j,y_j), y_j ; d_i)]$. Colloquially $r_{d_i, a_i}$ represents the expected robustness of defense $d_i$ when evaluating adversarial samples generated by attack $a_i$. From a game theoretic perspective, $r_{d,a}$ is the payoff for $p_D$ when they play strategy $d$ and $p_A$ plays strategy $a$. The payoff for $p_A$ given strategies $d,a$ is $-r_{d,a}$. Our mini-max optimization problem can then be simplified to:
\begin{equation}
   \displaystyle  \min_{\lambda^D} \max_{\lambda^A} \sum_{a_i \in A} \lambda^A_i \sum_{d_i \in D} \lambda^D_i r_{d_i, a_i}
\end{equation}
From this we can create a finite, tabular, zero-sum game defined by the following game-frame in strategic form:
\begin{equation}
    \langle \{p_A, p_D\}, \; (A,D), \; O, \; f \rangle
\end{equation}
where $O = \{ r_{d,a} \; \forall a \in A, \; d \in D \}$ and $f$ is a function $f : A \times D \rightarrow O$ defined by $f(d,a) = r_{d,a}$. Because this is a finite, tabular, zero-sum game, it has a Nash-Equilibrium~\cite{Nash}. Let $R$ be the payoff matrix for $p_D$ where $R_{d,a} = r_{d,a}$. It then becomes the goal of $p_D$ to maximize their guaranteed, expected payoff. Formally, $p_D$ must solve the following optimization problem:
\begin{equation}
\begin{array}{c c}
    \displaystyle \max_{r^* ; \lambda^D} r^* \,  & \text{subject to } \lambda^D R \geq (r^*, \cdots r^*) \text{ and } ||\lambda^D||_1 \leq 1
\end{array}
\end{equation}
This optimization problem is a linear program, the explicit form of which we provide in the supplemental material. All linear programs have a dual problem, in this case the dual problem finds a mixed Nash strategy for $p_A$. This can be done by changing the problem to a minimization problem and transposing $R$. In the interest of space we give the explicit form of the dual problem in the supplemental material as well. These linear programs can be solved using polynomial time algorithms. 
\subsection{$\textbf{GaME}_n$}
$\text{GaME}_n$ is a more general family of games of which $\text{GaME}_1$ is a special case. In $\text{GaME}_n$, for $n>1$, $p_D$ can calculate their final prediction based upon the output logits of multiple $d \in D$ evaluated on the same input $x$. For this to occur, $p_D$ must also choose a function to map the output of multiple defenses to a final prediction. Formally, the strategy set of $p_D$ becomes $D = D' \times F$, where $F$ is a set of prediction functions and $D'$ is defined as follows.
\begin{equation}
    D' \subseteq \{U : U \subseteq D, \; |U| \leq n\}
\end{equation}
Multi-model prediction functions can increase the overall robustness of an ensemble by requiring an adversarial sample to be misclassified by multiple models simultaneously~\cite{BARZ}. In this paper we focus on two voting functions: the majority vote ($f^h$)~\cite{BaRT}, and the largest softmax probability vote ($f^s$)~\cite{demystifying}:% We will refer to these as $f^h$ and $f^s$ respectively:
\begin{equation}
    f^h(x, U) = \displaystyle \argmax_{y \in \mathcal{Y}} \sum_{d \in U} \mathbbm{1} \{ y = \argmax_{j \in \mathcal{Y}} d_j(x)\}
    \label{eq:fh}
\end{equation}
\begin{equation}
    f^s(x, U) = \displaystyle \argmax_{y \in \mathcal{Y}} \frac{1}{|U|} \sum_{d \in U} \sigma(d(x))
    \label{eq:fs}
\end{equation}
where $\mathbbm{1}$ is the indicator function, $\sigma$ is the softmax function, and $d_j(x)$ represents the $j^{th}$ output logit of defense $d$ when evaluated on input $x$. Solving $\text{GaME}_n$ is the same as solving $\text{GaME}_1$, except with larger $|D|$. Notationally, the mini-max optimization problem in terms of $r_{d,a}$ remains the same as we have simply redefined $D$, however we can redefine $r_{d,a}$ as follows:
\begin{equation}
    r_{(U_i, f_j), a_k} = \sum_{l=0}^N [L(x_l + a_k(x_l,y_l), y_l ; (U_i, f_j))]
\end{equation}
where $(U_i, f_j) \in D = D' \times F$. Similarly to $\text{GaME}_1$, in $\text{GaME}_n$  $r_{(U_i,f_j),a_k}$ represents the expected robust accuracy, i.e., the payoff, for $p_D$ if they play strategy $(U_i,f_j)$ and $p_A$ plays strategy $a_k$.
\subsection{$\textbf{GaME-D}_n$ and MAGE-D}
%Motivated by the findings of Section~\ref{sec:trans}, here we further build upon the GaME framework, allowing the defender to implement adversarial detection as a method for thwarting attacks. This new defense, $\text{GaME-D}_n$, primarily differs from $\text{GaME}_n$ through the inclusion of a new voting function for the defender designed to detect adversarial examples:
%\color{red}this is kind of ambiguous but I am not sure what is the best way to do it given the small column horizontal space.\color{black}
% \begin{equation}
% f^d(x, U) = \left\{ \begin{array}{c c}
%     null & \text{if cond}(y')  \\
%     \argmax_{y \in \mathcal{Y}}(y') & \text{otherwise}
% \end{array}    \right.
% \end{equation}
Motivated by the low transferability of adversarial examples, as shown in Section~\ref{sec:trans}, we enhance the GaME framework to include adversarial detection. We denote this expanded framework as $\text{GaME-D}_n$. In the expanded framework, the defender $p_{d}$ is allowed to output an additionally adversarial label, $\bot$. The condition for a successful adversarial attack conducted by $p_{a}$ is then: $( f^{d}(x_{adv},D) \neq y) \land ( f^{d}(x_{adv},D)\neq \bot)$ where $D$ is the set of defenses and $(x,y)$ is the clean input and correct class label used to generate $x_{adv}$. In our setup we empirical found plurality voting to provide the best trade-off between robustness and clean accuracy. The plurality voting utilized by $p_{d}$ is: 
\begin{equation}
\begin{array}{c}
f^d(x, U) = \left\{ \begin{array}{c c}
    y'_i & \text{if } \exists \; V_{y'_i} : \forall y'_j \neq y'_i, \; V_{y'_i} > V_{y'_j} \\ 
    \bot & \text{otherwise}
\end{array}    \right. \\
%\displaystyle \text{where } y'_k = \sum_{d \in U} \mathbbm{1} \{ y'_k = \argmax_{y \in \mathcal{Y}} d_y(x) \}
\end{array}
\end{equation}
where $V_{y'_i}$ represents the total number of votes for class label $y'_i$ and $\bot$ represents the adversarial class label. Under $\text{GaME-D}_n$, the defender optimizes $r_{(U_i, f_j), a_k}$ for both clean accuracy and robustness (e.g. without optimizing over clean accuracy $p_{d}$ can always output $\bot$, achieving $100\%$ robustness but $0\%$ clean accuracy). Therefore, for both $\text{GaME}_n$ and $\text{GaME-D}_n$, we adjust the set of attacks $A$ such that $f^{identity} \in A$ where $f^{identity} : \mathcal{X} \times \mathcal{Y} \rightarrow P_{\epsilon, \mathcal{X}}$ defined by $ f^{identity}(x,y) = x$. 
\begin{algorithm}
\caption{MAGE} \label{alg:MAGE}
\begin{algorithmic}
\State {\textbf{Input}: clean sample $x$, true label $y$, boolean $targeted$.} 
\State \textbf{Initialize}: $G_{blend} = \hat{0}$ 
\State \textbf{Define}: $g(m, x) = \sum_{j=0}^{N_{samp}} \frac{\partial L_{m}}{\partial t_m(x_{adv}^{(i)})}$
\State \textbf{For} $i$ in range 1 to $N_{iter}$ do:
\State \hspace{10pt} $G_{blend} = \gamma \cdot G_{blend} + (\sum_{m=1}^{M}\alpha_{m}^{i}\odot g(m, x_{adv}^{(i)}) \odot \phi_{m})$
\State \hspace{10pt} \textbf{If} $targeted$
\State \hspace{20pt} $x_{adv}^{(i+1)}=x_{adv}^{(i)}-\epsilon_{step}\text{sign}(G_{blend})$
\State \hspace{10pt} \textbf{else}
\State \hspace{20pt} $x_{adv}^{(i+1)}=x_{adv}^{(i)}+\epsilon_{step}\text{sign}(G_{blend})$
\State \hspace{10pt} $x_{adv}^{i+1}=p(x_{adv}^{(i)}, x, \epsilon_{max})$
\State \hspace{10pt} \textbf{For} $m$ in range 1 to M:
\State \hspace{20pt}${\frac{\partial x_{adv}^{(i)}}{\partial \alpha _{m}^{(i)}}} \approx u\epsilon _{step} \text{sech}^{2}(u\sum_{m=1}^{M}  g(m, x_{adv}^{(i)}) \odot $
\State \hspace{50pt} $g(m, x_{adv}^{(i)}))$
\State \hspace{20pt}${\frac{\partial F}{\partial \alpha _{m}^{(i)}}}=
{\frac{\partial F}{\partial \alpha _{adv}^{(i)}}}\odot 
\frac{\partial x_{adv}^{(i)}}{\partial \alpha _{m}^{(i)}}$
\State \hspace{20pt}$\alpha _{m}^{(i)}=\alpha _{m}^{(i)}-r{\frac{\partial F}{\partial \alpha _{m}^{(i)}}}$
\State \hspace{10pt} end for
\State  end for
\State {\textbf{Output}:} $x_{adv}$
\end{algorithmic}
\end{algorithm} 
\begin{algorithm}
\caption{MAGE-D}\label{alg:MAGE-D}
\begin{algorithmic}
\State {\textbf{Input}: clean sample $x$, true label $y$.} 
\State \textbf{Let} $\sigma (m,x)$ be a function that gets the output logits of a classifier $m$ given input $x$
\State \textbf{Initialize} $y_{adv}$, $x'_{adv}$, and $s$ to be lists indexed by $m \in M$
\State $x_{adv}$ = MAGE($x$, $y$, False)
\State \textbf{If} $D(x_{adv}) \neq y$ and $D(x_{adv}) \neq null$
    \State \hspace{10pt} \textbf{return} $x_{adv}$
\State \textbf{For} $m \in M$
    \State \hspace{10pt} $y'_{m} = m(x_{adv})$
    \State \hspace{10pt} \textbf{If} $y' \neq y$
        \State \hspace{20pt} $x'_{adv, m} =$ MAGE($x$, $y'_m$, True)
        \State \hspace{20pt} $s_m = \sigma(D, x'_{adv, m})$
\State  $m^* = \argmax_{m \in M} [\max_{y'} s_{m, y' \neq y}]$
\State \textbf{return} $x'_{adv,m^*}$
\end{algorithmic}
\end{algorithm}
MAGE, MIME, and APGD, are agnostic to the adversarial detection defenses. To represent a stronger adversary, we propose a modification to the MAGE attack, MAGE-D. The attack exploits a key property of the detector's voting scheme: by leveraging a targeted version of MAGE, the attacker can work to achieve a plurality of votes for the wrong class label. A detailed description of the algorithm can be found in Algorithms~\ref{alg:MAGE} and~\ref{alg:MAGE-D}. For this attack, we define the attack parameters as follows: number of iterations $N_{iter}$, number of samples $N_{samp}$, step size per iteration $\epsilon_{iter}$, maximum perturbation  $\epsilon_{max}$, coefficient learning rate $r$, and detector, $D$, utilizing a set of models, $M$, with corresponding loss functions $L_{m_1},..,L_{m_{|M|}}$ and transform functions $t_{m_1},...,t_{m_{|M|}}$. Additionally we utilize a projection function $p: \mathcal{X} \rightarrow P_{\epsilon_{max}, \mathcal{X}}$ which projects an adversarial example, $x_{adv}$, generated from clean sample, $x$, such that $|x_{adv} - x|_\infty \leq \epsilon_{max}$.

MAGE-D is able to increase the attack success rate of MAGE by 50\% on CIFAR-10 and 85.3\% on Tiny ImageNet when attacking a detector utilizing vanilla voting models. Further details for these results can be found in the supplementary material.


%to fool it, one must convince a plurality of the voting models to produce the same, incorrect class label. Therefore MAGE-D utilizes targeted attacks to convince each model in the detector to predict the same class label.



%****This is no longer true****
%Since MAGE-D is specifically designed to attack our proposed GaME and GaME-D defenses, we will not include the attack in our optimization problem. This allows us to test the robustness of our defense against attacks it has not optimized over, dispelling worries over false robustness. These results will be explored in more detail in the following section.

%The size of $D'$ can grow exponentially in $|D|$, which can dramatically increase the computational complexity of calculating the payoff matrix, $R$. However, once each 



%All of this is a more complex say of saying what is above
%where $\lambda^A$ and $\lambda^D$ represent the mixed strategies of $p_A$ and $p_D$ respectively. For convenience we will let each, unique $a_i \in A$ correspond to the $i^{th}$ element of $\lambda^A$, $\lambda^A_i$, and will do the same for each, unique $d_i \in D$ by letting it correspond to the $i^{th}$ element of $\lambda^D$, $\lambda^D_i$. Additionally, without loss of generality, we will assume that each $\lambda^A$, $\lambda^D$ are organized such that $\lambda^A_{i-1} \leq \lambda^A_{i-1}$, and $\lambda^D_{i-1} \leq \lambda^D_{i-1} $. We can then define the following push forward from each $\lambda^A$, $\lambda^D$ to $A,D$:

%\begin{equation}
%    \mathbb{P}(\{a_i \in A : a = a_i\}) = \left\{ \begin{array}{c c}
%        \mathbb{P}(\{r \in R^+ : \lambda^A_{i-1} < r\}) & \text{ if } i = |A| \\
%        \mathbb{P}(\{r \in R^+ : r \leq \lambda^A_{i-1} \}) & \text{ if } i = 0 \\
%        \mathbb{P}(\{r \in R^+ : \lambda^A_{i-1} < r \leq \lambda^A_{i-1} \}) & \text{ if } 0 < i < |A| 
%    \end{array} \right.
%\end{equation}

%A null output is considered a correct prediction if and only if the original input was an adversarial example. Thus the defender's loss function must be adjusted accordingly when calculating $r_{(U_i, f_j), a_k}$. One concern with this setup is that the GaME algorithm may choose a mixed strategy that prioritizes detectors with a high chance of producing a null label. This will cause the robust accuracy of the defense to be high while causing the clean accuracy to decrease significantly. Therefore, for both $\text{GaME}_n$ and $\text{GaME-D}_n$, we adjust the set of attacks $A$ such that $f^{identity} \in A$ where $f^{identity} : \mathcal{X} \times \mathcal{Y} \rightarrow P_{\epsilon, \mathcal{X}}$ defined by $ f^{identity}(x,y) = x$. This allows the defender to optimize over robust accuracy in addition to clean accuracy within the GaME framework. 
%, and cond$(y')$ is a condition that is true when $\exists y'_j, \, y'_i \; s.t. \; y'_j = y'_i = \max(y'), \; j \neq i$
%where $y'$ is a vector with elements $y'_i = \sum_{d \in U} \mathbbm{1} \{ y'_i = \argmax_{y \in \mathcal{Y}} d_y(x)$.
%Since the previously discussed attacks were untargeted it is possible, if not likely, that the attack moved each model to predict different class labels, causing the detector to output a null class label.
%\color{red} While it is possible for one attack the detector with an attack which exhaustively tries each possible, incorrect class label, this becomes intractable for data sets with a large number of class labels such as Image Net. Therefore we propose MAGE-D as a way of shrinking the search space of incorrect class labels such that it scales linearly with the number of models in the detector and is constant in the total number of possible class labels. \color{black}

%It does this through a multi-stage process: first attacking the detector with the untargeted MAGE attack. From the generated sample each model in the detector will produce a class label. For each incorrect class label produced, $y'$, we will attack the detector again with a targeted MAGE attack, using $y'$ as the target label. $y'$ is chosen as the target since we know at least one of the models in the detector is already vulnerable to producing that incorrect label. Thus, we try to move the rest of the models to produce that same, incorrect label. For each of the targeted attacks we choose the generated sample which produces the highest confidence of an incorrect class label in the detector. A more detailed description of the algorithm can be found in Algorithms~\ref{alg:MAGE} and~\ref{alg:MAGE-D}.

==> GaME E-Print V2/Sections/Introduction.tex <==


\section{Introduction}
%Say classify too much
As Machine Learning models are continually integrated into safety critical regions of the digital and physical world it becomes ever more important to understand and mitigate their security weaknesses. While high complexity models such as CNNs and Vision Transformers are able to achieve high levels of accuracy in the image classification domain, they remain susceptible to misclassifying images modified by an adversary. These images, commonly referred to as adversarial examples, are easily classified by a human, but contain small perturbations that can lead to arbitrary misclassifications by state-of-the-art classifiers as determined by the adversary.

Due to this security threat, the study of adversarial examples, Adversarial Machine Learning, has become a rapidly developing field, with new defense architectures and attack techniques being published regularly. Many of these defenses achieve state-of-the-art levels of robustness against adversarial examples generated by standard attacks, but are eventually broken by an attack specifically designed to target their weaknesses. For instance, randomized defenses such as BaRT~\cite{BaRT} and Trash is Treasure~\cite{TiT} can be targeted by Expectation over Transformation attacks (EOT)~\cite{EOT}; while models trained with Adversarial Training techniques such as Friendly Adversarial Training (FAT)~\cite{FAT} are often susceptible to sufficiently strong white box attacks such as the Adaptive Projected Gradient Descent (APGD)~\cite{APGD}. 

Recent works have theoretically and empirically demonstrated a need for the implementation of ensemble defenses to mitigate the effects of adversarial examples~\cite{araujo2020advocating}. To this end, others have developed new techniques for adversarially training ensemble defenses~\cite{pinot2020randomization} and have additionally analyzed Adversarial Training and Adversarial Machine Learning in a Game Theoretic context. ~\cite{meunier2021mixed} in particular demonstrates the existence of a Nash Equilibrium in the adversarial examples game, one in which the defender and attacker can both choose mixed strategies. In addition to signaling a need for randomized ensemble defenses, these papers illustrate a need for randomized ensemble attacks to counter them. Motivated by this we propose a new, practical framework for finding the Nash Equilibrium of the adversarial examples game played between an attacker and defender who both have access to a set of state-of-the-art adversarial attacks and defenses respectively.

%Mention the transfer study between defenses
In addition to this we 

==> GaME E-Print V2/Sections/Introduction2.tex <==
\section{Introduction}

Machine learning models have been shown to be vulnerable to adversarial examples~\cite{goodfellow2014explaining, papernot2016transferability}. Adversarial examples are inputs with small perturbations added, such that machine learning models misclassify them with high confidence. Addressing the security risks posed by adversarial examples are critical for the safe deployment of machine learning in areas like health care~\cite{medicineAdvML} and self driving vehicles~\cite{drivingAdvML}. However, current defenses and attacks in adversarial machine learning have trended towards a cat and mouse dynamic, where in new defenses are being proposed and then broken~\cite{bypassing10detectors, tramer2020adaptive, mahmood2021beware, demystifying} by improved attacks.  

In parallel to attack and defense development, studies have also been conducted on the transferability of adversarial examples~\cite{Delving, mahmood2021robustness, xu2022securing}. Transferabiltiy refers to the phenomena where adversarial examples generated for one model are also misclassified by a different machine learning model. However, to the best of our knowledge no analyses have been done on the transferability of adversarial examples designed to attack specific defenses. From these observations several pertinent questions arise:
\begin{enumerate}
    \item \textit{Do adversarial examples generated for one specific defense transfer to other defenses?}
    \item \textit{Based on adversarial transferability, can a game theoretic framework be developed to determine the optimal choices for both attacker and defender?}
    \item \textit{How can the addition of multi-defense consensus voting (adversarial detection) and multi-model attacks be exploited by both the attacker and defender within a game theoretic framework?}
\end{enumerate}
These are precisely the questions our paper seeks to answer. We break from the traditional dynamic of adversarial machine learning, which focuses on the single best attack and defense. We instead take a multi-faceted approach and develop a game theoretic framework to answer the above questions. We provide the following contributions: 
\begin{enumerate}
    \item \textbf{Defense Transferability Analysis}- We analyze the adversarial transferability of state-of-the-art defenses like Trash is Treasure~\cite{TiT}, Barrage of Random Transforms~\cite{BaRT}, Friendly Adversarial Training~\cite{FAT} and other new architectures like SNNs~\cite{transferSNN, SEW} and ViTs~\cite{VIT}. We show specific attacks on defenses do no transfer well, meaning there is potential for a combinational defense within a game theoretic framework.
    \item \textbf{New Combinational Adversarial Attacks} - We develop three new attacks: the Momentum Iterative Method over Expectation attack (MIME), the Multi-Agent Gradient Expectation attack (MAGE) and detector based Multi-Agent Gradient Expectation attack (MAGE-D). These attacks are designed to create the strongest possible adversary to attack randomized and multi-classifier based defenses.  
    \item \textbf{Game theoretic Mixed Experts} - We propose a game-theoretic framework for finding approximately optimal strategies for adversarial attackers and defenders that can implement multi-model attack and defense techniques. We mathematically derive our framework, and empirical test it  by implementing multiple state-of-the-art adversarial attacks and defenses on two datasets, CIFAR-10~\cite{c10} and Tiny ImageNet~\cite{le2015tiny}. Through our framework we demonstrate that we are able to achieve a 37.3\% increase in robustness on CIFAR-10, and a 45.65\% increase on Tiny ImageNet over all single-model defenses we tested. 
\end{enumerate}

%We show we can accomplish this while maintaining a high level of accuracy on unperturbed images.

%Most importantly, we formulate a practical, game-theoretic framework for finding the optimal strategies for an attacker and defender who each employ a set of state-of-the-art adversarial attacks and defenses. Motivated by this framework, and in order to create a stronger adversary, we develop three new white-box attacks. We develop the Momentum Iterative Method over Expectation attack (MIME) for randomized defenses. For multi-model classifiers based defenses we synthesize the Multi-Agent Gradient Expectation attack (MAGE) and for detectors we craft MAGE-D. These attacks are necessary for targeting certain randomized defenses and for adapting to multi-defense strategies. Lastly, we analyze the adversarial transferability of current defenses like Trash is Treasure~\cite{TiT}, Barrage of Random Transforms~\cite{BaRT}, Friendly Adversarial Training~\cite{FAT} and other new architectures like SNNs~\cite{transferSNN, SEW} and ViTs~\cite{VIT}. We further leverage the low transferability between these classifiers to find those which are best suited for a combined, ensemble defense such as the one developed in our game-theoretic framework. 

In contrast to previous works studying similar adversarial games~\cite{sengupta2018mtdeep}, our framework is more comprehensive, state-of-the-art, and includes broader analyses. Specifically, we consider an adversary that can employ both state-of-the-art single model and multi-model attacks (of which we formulate three new ones). Likewise, our defender is different from~\cite{sengupta2018mtdeep} in that they can utilize randomized transformations, different voting schemes, and adversarial detection mechanisms. Overall, our paper demonstrates that by using our framework, higher robustness can be achieved than any single state-of-the art defense we studied. %We further separate ourselves by formulating three new, unique adversarial attacks specifically designed to target the weaknesses of our defense model and by studying the adversarial transferability between different defense architectures. 
%These are precisely the questions our paper seeks to answer. We break from the traditional dynamic of adversarial machine learning which focuses on the single best attack and defense. We instead take a multi-faceted approach and develop a game theoretic framework to answer the above questions. Specifically, we provide the following contributions: On the attack side we develop two new white-box attacks called the Momentum Iterative Method over Expectation (MIME) and the Auto Expectation Self-Attention Gradient Attack (AE-SAGA). These attacks are necessary for targeting certain randomized defenses and for adapting to multi-defense strategies. We analyze the adversarial transferability of current defenses like Trash is Treasure~\cite{TiT}, Barrage of Random Transforms~\cite{BaRT}, Friendly Adversarial Training~\cite{FAT} and other new architectures like SNNs~\cite{transferSNN, SEW} and ViTs~\cite{VIT}. Lastly, and most importantly, we formulate a practical, game-theoretic framework for finding the optimal strategies for an attacker and defender who each employ a set of state-of-the-art adversarial attacks and defenses. %This framework allows both parties to improve their expected attack success rate and robust accuracy respectively.


==> Sections/Introduction.tex <==


\section{Introduction}
%Say classify too much
As Machine Learning models are continually integrated into safety critical regions of the digital and physical world it becomes ever more important to understand and mitigate their security weaknesses. While high complexity models such as CNNs and Vision Transformers are able to achieve high levels of accuracy in the image classification domain, they remain susceptible to misclassifying images modified by an adversary. These images, commonly referred to as adversarial examples, are easily classified by a human, but contain small perturbations that can lead to arbitrary misclassifications by state-of-the-art classifiers as determined by the adversary.

Due to this security threat, the study of adversarial examples, Adversarial Machine Learning, has become a rapidly developing field, with new defense architectures and attack techniques being published regularly. Many of these defenses achieve state-of-the-art levels of robustness against adversarial examples generated by standard attacks, but are eventually broken by an attack specifically designed to target their weaknesses. For instance, randomized defenses such as BaRT~\cite{BaRT} and Trash is Treasure~\cite{TiT} can be targeted by Expectation over Transformation attacks (EOT)~\cite{EOT}; while models trained with Adversarial Training techniques such as Friendly Adversarial Training (FAT)~\cite{FAT} are often susceptible to sufficiently strong white box attacks such as the Adaptive Projected Gradient Descent (APGD)~\cite{APGD}. 

Recent works have theoretically and empirically demonstrated a need for the implementation of ensemble defenses to mitigate the effects of adversarial examples~\cite{araujo2020advocating}. To this end, others have developed new techniques for adversarially training ensemble defenses~\cite{pinot2020randomization} and have additionally analyzed Adversarial Training and Adversarial Machine Learning in a Game Theoretic context. ~\cite{meunier2021mixed} in particular demonstrates the existence of a Nash Equilibrium in the adversarial examples game, one in which the defender and attacker can both choose mixed strategies. In addition to signaling a need for randomized ensemble defenses, these papers illustrate a need for randomized ensemble attacks to counter them. Motivated by this we propose a new, practical framework for finding the Nash Equilibrium of the adversarial examples game played between an attacker and defender who both have access to a set of state-of-the-art adversarial attacks and defenses respectively.

%Mention the transfer study between defenses
In addition to this we 
